Making Code Re-randomization Practical with MARDU

Defense techniques such as Data Execution Prevention (DEP) and Address Space Layout Randomization (ASLR) were the early role models preventing primitive code injection and return-oriented programming (ROP) attacks. Notably, these techniques did so in an elegant and utilitarian manner, keeping performance and scalability in the forefront, making them one of the few widely-adopted defense techniques. As code re-use has evolved in complexity from JIT-ROP, to BROP and data-only attacks, defense techniques seem to have tunneled on defending at all costs, losing-their-way in pragmatic defense design. Some fail to provide comprehensive coverage, being too narrow in scope, while others provide unrealistic overheads leaving users willing to take their chances to maintain performance expectations. We present Mardu, an on-demand system-wide re-randomization technique that improves re-randomization and refocuses efforts to simultaneously embrace key characteristics of defense techniques: security, performance, and scalability. Our code sharing with diversification is achieved by implementing reactive and scalable, rather than continuous or one-time diversification while the use of hardware supported eXecute-only Memory (XoM) and shadow stack prevent memory disclosure; entwining and enabling code sharing further minimizes needed tracking, patching costs, and memory overhead. Mardu's evaluation shows performance and scalability to have low average overhead in both compute-intensive (5.5% on SPEC) and real-world applications (4.4% on NGINX). With this design, Mardu demonstrates that strong and scalable security guarantees are possible to achieve at a practical cost to encourage deployment.

==> code/fmt.tex <==

\makeatletter
\def\PY@reset{\let\PY@it=\relax \let\PY@bf=\relax%
    \let\PY@ul=\relax \let\PY@tc=\relax%
    \let\PY@bc=\relax \let\PY@ff=\relax}
\def\PY@tok#1{\csname PY@tok@#1\endcsname}
\def\PY@toks#1+{\ifx\relax#1\empty\else%
    \PY@tok{#1}\expandafter\PY@toks\fi}
\def\PY@do#1{\PY@bc{\PY@tc{\PY@ul{%
    \PY@it{\PY@bf{\PY@ff{#1}}}}}}}
\def\PY#1#2{\PY@reset\PY@toks#1+\relax+\PY@do{#2}}

\expandafter\def\csname PY@tok@w\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.73,0.73}{##1}}}
\expandafter\def\csname PY@tok@c\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.74,0.48,0.00}{##1}}}
\expandafter\def\csname PY@tok@k\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.69,0.00,0.25}{##1}}}
\expandafter\def\csname PY@tok@o\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@ow\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@nb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@nc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@nn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@ne\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.82,0.25,0.23}{##1}}}
\expandafter\def\csname PY@tok@nv\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@no\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@nl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@ni\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.60,0.60,0.60}{##1}}}
\expandafter\def\csname PY@tok@na\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.49,0.56,0.16}{##1}}}
\expandafter\def\csname PY@tok@nt\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@s\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sd\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@si\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@se\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.13}{##1}}}
\expandafter\def\csname PY@tok@sr\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@ss\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@sx\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@m\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@gh\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@gu\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.50,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@gd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@gi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@gr\endcsname{\def\PY@tc##1{\textcolor[rgb]{1.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@ge\endcsname{\let\PY@it=\textit}
\expandafter\def\csname PY@tok@gs\endcsname{\let\PY@bf=\textbf}
\expandafter\def\csname PY@tok@gp\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@go\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.53,0.53}{##1}}}
\expandafter\def\csname PY@tok@gt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.27,0.87}{##1}}}
\expandafter\def\csname PY@tok@err\endcsname{\def\PY@bc##1{\setlength{\fboxsep}{0pt}\fcolorbox[rgb]{1.00,0.00,0.00}{1,1,1}{\strut ##1}}}
\expandafter\def\csname PY@tok@kc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kd\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kr\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@bp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@fm\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@vc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vg\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vm\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@sa\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@dl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@s2\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@s1\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@mb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@il\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mo\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@ch\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cm\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cpf\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@c1\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cs\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}

\def\PYZbs{\char`\\}
\def\PYZus{\char`\_}
\def\PYZob{\char`\{}
\def\PYZcb{\char`\}}
\def\PYZca{\char`\^}
\def\PYZam{\char`\&}
\def\PYZlt{\char`\<}
\def\PYZgt{\char`\>}
\def\PYZsh{\char`\#}
\def\PYZpc{\char`\%}
\def\PYZdl{\char`\$}
\def\PYZhy{\char`\-}
\def\PYZsq{\char`\'}
\def\PYZdq{\char`\"}
\def\PYZti{\char`\~}
% for compatibility with earlier versions
\def\PYZat{@}
\def\PYZlb{[}
\def\PYZrb{]}
\makeatother



==> data/bruteforce-rerand.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\scriptsize
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5040.00,1440.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(381,143){\makebox(0,0)[r]{\strut{}0}}%
      \csname LTb\endcsname%
      \put(381,271){\makebox(0,0)[r]{\strut{}2}}%
      \csname LTb\endcsname%
      \put(381,399){\makebox(0,0)[r]{\strut{}4}}%
      \csname LTb\endcsname%
      \put(381,527){\makebox(0,0)[r]{\strut{}6}}%
      \csname LTb\endcsname%
      \put(381,655){\makebox(0,0)[r]{\strut{}8}}%
      \csname LTb\endcsname%
      \put(381,783){\makebox(0,0)[r]{\strut{}10}}%
      \csname LTb\endcsname%
      \put(381,911){\makebox(0,0)[r]{\strut{}12}}%
      \csname LTb\endcsname%
      \put(381,1039){\makebox(0,0)[r]{\strut{}14}}%
      \csname LTb\endcsname%
      \put(381,1167){\makebox(0,0)[r]{\strut{}16}}%
      \csname LTb\endcsname%
      \put(381,1295){\makebox(0,0)[r]{\strut{}18}}%
      \csname LTb\endcsname%
      \put(584,71){\rotatebox{45}{\makebox(0,0)[r]{\strut{}1000ms}}}%
      \csname LTb\endcsname%
      \put(846,71){\rotatebox{45}{\makebox(0,0)[r]{\strut{}100ms}}}%
      \csname LTb\endcsname%
      \put(1108,71){\rotatebox{45}{\makebox(0,0)[r]{\strut{}50ms}}}%
      \csname LTb\endcsname%
      \put(1370,71){\rotatebox{45}{\makebox(0,0)[r]{\strut{}10ms}}}%
      \csname LTb\endcsname%
      \put(1632,71){\rotatebox{45}{\makebox(0,0)[r]{\strut{}1ms}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(163,719){\rotatebox{-270}{\makebox(0,0){\strut{}Performance overhead (\%)}}}%
      \put(1000,1475){\makebox(0,0){\strut{}milc}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1994,143){\makebox(0,0)[r]{\strut{}0}}%
      \csname LTb\endcsname%
      \put(1994,271){\makebox(0,0)[r]{\strut{}2}}%
      \csname LTb\endcsname%
      \put(1994,399){\makebox(0,0)[r]{\strut{}4}}%
      \csname LTb\endcsname%
      \put(1994,527){\makebox(0,0)[r]{\strut{}6}}%
      \csname LTb\endcsname%
      \put(1994,655){\makebox(0,0)[r]{\strut{}8}}%
      \csname LTb\endcsname%
      \put(1994,783){\makebox(0,0)[r]{\strut{}10}}%
      \csname LTb\endcsname%
      \put(1994,911){\makebox(0,0)[r]{\strut{}12}}%
      \csname LTb\endcsname%
      \put(1994,1039){\makebox(0,0)[r]{\strut{}14}}%
      \csname LTb\endcsname%
      \put(1994,1167){\makebox(0,0)[r]{\strut{}16}}%
      \csname LTb\endcsname%
      \put(1994,1295){\makebox(0,0)[r]{\strut{}18}}%
      \csname LTb\endcsname%
      \put(2197,71){\rotatebox{45}{\makebox(0,0)[r]{\strut{}1000ms}}}%
      \csname LTb\endcsname%
      \put(2459,71){\rotatebox{45}{\makebox(0,0)[r]{\strut{}100ms}}}%
      \csname LTb\endcsname%
      \put(2721,71){\rotatebox{45}{\makebox(0,0)[r]{\strut{}50ms}}}%
      \csname LTb\endcsname%
      \put(2983,71){\rotatebox{45}{\makebox(0,0)[r]{\strut{}10ms}}}%
      \csname LTb\endcsname%
      \put(3245,71){\rotatebox{45}{\makebox(0,0)[r]{\strut{}1ms}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(2613,1475){\makebox(0,0){\strut{}sjeng}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(3607,143){\makebox(0,0)[r]{\strut{}0}}%
      \csname LTb\endcsname%
      \put(3607,271){\makebox(0,0)[r]{\strut{}2}}%
      \csname LTb\endcsname%
      \put(3607,399){\makebox(0,0)[r]{\strut{}4}}%
      \csname LTb\endcsname%
      \put(3607,527){\makebox(0,0)[r]{\strut{}6}}%
      \csname LTb\endcsname%
      \put(3607,655){\makebox(0,0)[r]{\strut{}8}}%
      \csname LTb\endcsname%
      \put(3607,783){\makebox(0,0)[r]{\strut{}10}}%
      \csname LTb\endcsname%
      \put(3607,911){\makebox(0,0)[r]{\strut{}12}}%
      \csname LTb\endcsname%
      \put(3607,1039){\makebox(0,0)[r]{\strut{}14}}%
      \csname LTb\endcsname%
      \put(3607,1167){\makebox(0,0)[r]{\strut{}16}}%
      \csname LTb\endcsname%
      \put(3607,1295){\makebox(0,0)[r]{\strut{}18}}%
      \csname LTb\endcsname%
      \put(3810,71){\rotatebox{45}{\makebox(0,0)[r]{\strut{}1000ms}}}%
      \csname LTb\endcsname%
      \put(4072,71){\rotatebox{45}{\makebox(0,0)[r]{\strut{}100ms}}}%
      \csname LTb\endcsname%
      \put(4334,71){\rotatebox{45}{\makebox(0,0)[r]{\strut{}50ms}}}%
      \csname LTb\endcsname%
      \put(4595,71){\rotatebox{45}{\makebox(0,0)[r]{\strut{}10ms}}}%
      \csname LTb\endcsname%
      \put(4857,71){\rotatebox{45}{\makebox(0,0)[r]{\strut{}1ms}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4225,1475){\makebox(0,0){\strut{}gobmk}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{data/bruteforce-rerand}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> data/nginx.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\scriptsize
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4752.00,1872.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(516,384){\makebox(0,0)[r]{\strut{}0}}%
      \csname LTb\endcsname%
      \put(516,653){\makebox(0,0)[r]{\strut{}500}}%
      \csname LTb\endcsname%
      \put(516,921){\makebox(0,0)[r]{\strut{}1000}}%
      \csname LTb\endcsname%
      \put(516,1190){\makebox(0,0)[r]{\strut{}1500}}%
      \csname LTb\endcsname%
      \put(516,1458){\makebox(0,0)[r]{\strut{}2000}}%
      \csname LTb\endcsname%
      \put(516,1727){\makebox(0,0)[r]{\strut{}2500}}%
      \csname LTb\endcsname%
      \put(1103,264){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%
      \put(1789,264){\makebox(0,0){\strut{}$8$}}%
      \csname LTb\endcsname%
      \put(2476,264){\makebox(0,0){\strut{}$12$}}%
      \csname LTb\endcsname%
      \put(3162,264){\makebox(0,0){\strut{}$16$}}%
      \csname LTb\endcsname%
      \put(3849,264){\makebox(0,0){\strut{}$20$}}%
      \csname LTb\endcsname%
      \put(4535,264){\makebox(0,0){\strut{}$24$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(96,1055){\rotatebox{-270}{\makebox(0,0){\strut{}Bandwidth (MB/sec)}}}%
      \put(2561,84){\makebox(0,0){\strut{}\# of worker processes}}%
      \csname LTb\endcsname%
      \put(1164,1589){\makebox(0,0)[r]{\strut{}\sys}}%
      \csname LTb\endcsname%
      \put(1164,1439){\makebox(0,0)[r]{\strut{}Vanilla}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{data/nginx}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> data/scalability.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\scriptsize
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4752.00,2160.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(300,384){\makebox(0,0)[r]{\strut{}0}}%
      \csname LTb\endcsname%
      \put(300,792){\makebox(0,0)[r]{\strut{}2}}%
      \csname LTb\endcsname%
      \put(300,1200){\makebox(0,0)[r]{\strut{}4}}%
      \csname LTb\endcsname%
      \put(300,1607){\makebox(0,0)[r]{\strut{}6}}%
      \csname LTb\endcsname%
      \put(300,2015){\makebox(0,0)[r]{\strut{}8}}%
      \csname LTb\endcsname%
      \put(372,264){\makebox(0,0){\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(1066,264){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%
      \put(1760,264){\makebox(0,0){\strut{}$8$}}%
      \csname LTb\endcsname%
      \put(2454,264){\makebox(0,0){\strut{}$12$}}%
      \csname LTb\endcsname%
      \put(3147,264){\makebox(0,0){\strut{}$16$}}%
      \csname LTb\endcsname%
      \put(3841,264){\makebox(0,0){\strut{}$20$}}%
      \csname LTb\endcsname%
      \put(4535,264){\makebox(0,0){\strut{}$24$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(96,1199){\rotatebox{-270}{\makebox(0,0){\strut{}Re-randomization latency (ms)}}}%
      \put(2453,84){\makebox(0,0){\strut{}\# of worker processes}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{data/scalability}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> tbl/adopted.tex <==
\begin{tabular}{llcccc}
  \toprule
  {\bf Mechanism} &
  {\bf Security Guarantees} &
  {\bf Perf.} &
  {\bf Worst} &
  {\bf Mem.} &
  {\bf CPU}
  \\
  \midrule
  StackGuard~\cite{wagle:stackguard}  &  seq. stack overflow       & <1\%           & 4\%          & {\bf N} & {\bf N} \\
  DEP~\cite{lwn:dep}                  &  shellcode execution       & $\approx$0\%   & $\approx$0\% & {\bf N} & {\bf N} \\
  ASLR~\cite{pax-aslr}                &  code reuse w/o leak       & $\approx$1\%   & 3\%          & {\bf N} & {\bf N} \\
  SafeStack~\cite{clang:safestack}    &  return address overwrite  & $\approx$0\%   & 4.1\%        & {\bf N} & {\bf N} \\
  CFI~\cite{clang:cfi}                &  indirect call/jump        & $\approx$5\%   & 8.7\%        & {\bf N} & {\bf N} \\
  \bottomrule
\end{tabular}


==> tbl/attack-surface-old.tex <==
    % ----------------------------------------------------------------------------
    % | Benchmark | Attack Surface                                        |  Coverage     |
    % |           | Call Instr | Indirect Call | PLT | #FN | # Ret | Total| SS |Trampoline|
    % =====================================================================================
    % | 400       |            |  X            |  X  |  X  |  X    |   O  | O  |    O     | 
    % | 401       |  O         |  X            |  X  |  X  |  X    |   O  | X  |    O     | 
    % | ..        |  O         |  X            |  X  |  X  |  X    |   O  | O  |    O     |
    % | 482       |  O         |  O            |  X  |  O  |  O    |   O  | O  |    O     |
    % ----------------------------------------------------------------------------
    % | NGINX     |  O         |  O            |  X  |  O  |  O    |   O  | O  |    O     |
    % ----------------------------------------------------------------------------
    % | MUSL      |  O         |  O            |  X  |  O  |  O    |   O  | O  |    O     |
    % 
% Variable declarations
\newcommand{\rIhI}{Benchmark}
\newcommand{\rIhII}{Attack Surface}
\newcommand{\rIhIII}{Mardu Coverage}
\newcommand{\rIhIV}{Residual}		% Residual attack surface

\newcommand{\rIIhI}{\#Call} 		% number of direct callsites
\newcommand{\rIIhII}{\#I-Call}	 	% Indirect Callsites
\newcommand{\rIIhIII}{\#Fn Entry}  	% number of function/function entries
\newcommand{\rIIhIV}{\#Ret Inst}   	% number of ret instr
\newcommand{\rIIhV}{\# Unintended C3}  	% number of other C3 opcode in code region
\newcommand{\rIIhVI}{Total Attack Sites}% SUM ^

\newcommand{\rIIhVII}{Mardu Coverage}
\newcommand{\rIIhVIII}{   \%}
\newcommand{\rIIhIX}{Remaining Sites}

\newcommand{\rowI}{perlbench}
\newcommand{\rowII}{bzip2}
\newcommand{\rowIII}{gcc}
\newcommand{\rowIV}{mcf}
\newcommand{\rowV}{milc}
\newcommand{\rowVI}{gobmk}
\newcommand{\rowVII}{hmmer}
\newcommand{\rowVIII}{sjeng}
\newcommand{\rowIX}{libquantum}
\newcommand{\rowX}{h264ref}
\newcommand{\rowXI}{lbm}
\newcommand{\rowXII}{sphinx3}
\newcommand{\rowXIII}{NGINX}
\newcommand{\rowXIV}{Musl Libc}
\newcommand{\rowXV}{Total}

\begin{tabular}{ll|rrrrr|r|rr|r}

  % first line
  \toprule
  	\multirow{2}{*} & {\textbf{\rIhI}} &
		\multicolumn{6}{c}{\textbf{\rIhII}} &
		\multicolumn{3}{c}{\textbf{\rIhIII}} \\ 
		%& \multicolumn{5}{c}{\textbf{\rIhIV}}\\
  	\cmidrule(r){3-9} & &
 		{\textbf{\rIIhI}} 	& {\textbf{\rIIhII}} 	& {\textbf{\rIIhIII}} & {\textbf{\rIIhIV}} &
  		{\textbf{\rIIhV}} 	& {\textbf{\rIIhVI}} 	& {\textbf{\rIIhVII}} & {\textbf{\rIIhVIII}} &
		{\textbf{\rIIhIX}}  \\

  \midrule
		%        Call      ICall #FN     #RET   Un C3  Total   Covered %Cove Remaining
  	\multirow{13}{*} &
	{\textbf{\rowI}} &13963    &272  &1668   &1854  &2390  &20147   &18479 &91.7 &1668 \\
	&{\textbf{\rowII}} &277	   &56   &81     &85    &98    &597     &516   &86.4 &81 \\
	&{\textbf{\rowIII}} &48096 &518  &4318   &5358  &5934  &64224   &59906 &93.3 &4318 \\
	&{\textbf{\rowIV}} &77     &3    &33     &33    &23    &169     &136   &80.5 &33 \\
	&{\textbf{\rowV}} &2104    &7    &244    &243   &294   &2892    &2648  &91.6 &244 \\
	&{\textbf{\rowVI}} &9521   &48   &2477   &2644  &1443  &16133   &13656 &84.6 &2477 \\
	&{\textbf{\rowVII}} &4237  &12   &478    &548   &737   &6012    &5534  &92.0 &478 \\
	&{\textbf{\rowVIII}} &1054 &4    &139    &175   &192   &1564    &1425  &91.1 &139 \\
	&{\textbf{\rowIX}} &469    &3    &107    &112   &69    &760     &653   &85.9 &107 \\
	&{\textbf{\rowX}} &3118    &372  &528    &570   &1243  &5831    &5303  &90.9 &528 \\
	&{\textbf{\rowXI}} &70     &3    &26     &25    &22    &146     &120   &82.2 &26 \\
	&{\textbf{\rowXII}} &2714  &11   &326    &345   &409   &3805    &3479  &91.4 &326 \\
	&{\textbf{\rowXIII}} &5316 &309  &1565   &1330  &867   &9387    &7822  &83.3 &1565 \\
	&{\textbf{\rowXIV}} &4400  &77   &3722   &1959  &1398  &11556   &7834  &67.8 &3722 \\
	&{\textbf{\rowXV}} &95416  &1695 &15712  &15281 &15119 &143223  &127511&89.0 &15712 \\

  \bottomrule
\end{tabular}




==> tbl/attack-surface.tex <==
\newcommand{\rowI}{perlbench}
\newcommand{\rowII}{bzip2}
\newcommand{\rowIII}{gcc}
\newcommand{\rowIV}{mcf}
\newcommand{\rowV}{milc}
\newcommand{\rowVI}{gobmk}
\newcommand{\rowVII}{hmmer}
\newcommand{\rowVIII}{sjeng}
\newcommand{\rowIX}{libquantum}
\newcommand{\rowX}{h264ref}
\newcommand{\rowXI}{lbm}
\newcommand{\rowXII}{sphinx3}
\newcommand{\rowXIII}{NGINX}
\newcommand{\rowXIV}{musl libc}
\newcommand{\rowXV}{Total}

\begin{tabular}{l|rr|rr|r|r}
  \toprule

  % first line
  \multirow{2}{*}{\textbf{Benchmark}} &
  \multicolumn{2}{c}{\textbf{Return address}} &
  \multicolumn{2}{c}{\textbf{ROP gadget}} &
  \textbf{Func reuse} &
  \textbf{\sys}
  \\
  \cmidrule(r){2-3}
  \cmidrule(r){4-5}
  \cmidrule(r){6-6}

  % second line
  &
  \textbf{\# \cc{call}} &
  \textbf{\# \cc{i-call}} &
  \textbf{\# \cc{ret}} &
  \textbf{\# \cc{u-ret}} &
  \textbf{\# fn entry} &
  \textbf{reduction (\%)}
  \\
  \midrule
	\textbf{\rowI}  &13963    &272   &1854  &2390  &1668  & 18479/20147 (91.7\%) \\
	\textbf{\rowII} &277	  &56    &85    &98    &81    & 516/597 (86.4\%) \\
	\textbf{\rowIII} &48096 &518     &5358  &5934 &4318   & 59906/64224 (93.3\%) \\
	\textbf{\rowIV} &77     &3       &33    &23   &33     & 136/169 (80.5\%) \\
	\textbf{\rowV} &2104    &7       &243   &294  &244    & 2648/2892 (91.6\%) \\
	\textbf{\rowVI} &9521   &48      &2644  &1443 &2477   & 13656/16133 (84.6\%) \\
	\textbf{\rowVII} &4237  &12      &548   &737  &478    & 5534/6012 (92.0\%) \\
	\textbf{\rowVIII} &1054 &4       &175   &192  &139    & 1425/1564 (91.1\%) \\
	\textbf{\rowIX} &469    &3       &112   &69   &107    & 653/760   (85.9\%) \\
	\textbf{\rowX} &3118    &372     &570   &1243 &528    & 5303/5831 (90.9\%) \\
	\textbf{\rowXI} &70     &3       &25    &22   &26     & 120/146   (82.2\%) \\
	\textbf{\rowXII} &2714  &11      &345   &409  &326    & 3479/3805 (91.4\%) \\
	\textbf{\rowXIII} &5316 &309     &1330  &867  &1565   & 7822/9387 (83.3\%) \\
	\textbf{\rowXIV} &4400  &77      &1959  &1398 &3722   & 7834/11556 (67.8\%) \\
  \midrule
	\textbf{\rowXV} &95416  &1695    &15281 &15119 &15712 & 127511/143223 (89.0\%) \\
  \bottomrule
\end{tabular}




==> tbl/sizes.tex <==
% Variable declarations
\newcommand{\firstColumn}{Benchmark}
\newcommand{\secondColumn}{Increases}
\newcommand{\subColumnI}{.text size increase}
\newcommand{\subColumnII}{Metadata size (bytes)}
\newcommand{\subColumnIII}{Trampolines count}
\newcommand{\rowI}{400.perlbench}
\newcommand{\rowII}{401.bzip2}
\newcommand{\rowIII}{403.gcc}
\newcommand{\rowIV}{429.mcf}
\newcommand{\rowV}{433.milc}
\newcommand{\rowVI}{445.gobmk}
\newcommand{\rowVII}{456.hmmer}
\newcommand{\rowVIII}{458.sjeng}
\newcommand{\rowIX}{462.libquantum}
\newcommand{\rowX}{464.h264ref}
\newcommand{\rowXI}{470.lbm}
\newcommand{\rowXII}{482.sphinx3}
\newcommand{\rowXIII}{NGINX}

\begin{tabular}{ll rrr}
	% Top of the table
	\toprule
		\multirow{2}[3]{*}{\bf \firstColumn} & \multicolumn{3}{c}{\bf \secondColumn}\\
		\cmidrule(ll){2-4} & & {\bf \subColumnI} & {\bf \subColumnII} & {\bf \subColumnIII}\\

	% Middle of the table
	\midrule
		\multicolumn{2}{l}{\rowI} & \the\numexpr\RESperlbench\relax & \the\numexpr\METAperlbench\relax & \the\numexpr\TOTALperlbench\relax\\
	\midrule
		\multicolumn{2}{l}{\rowII} & \the\numexpr\RESbzip\relax & \the\numexpr\METAbzip\relax & \the\numexpr\TOTALbzip\relax\\
	\midrule
		\multicolumn{2}{l}{\rowIII} & \the\numexpr\RESgcc\relax & \the\numexpr\METAgcc\relax & \the\numexpr\TOTALgcc\relax\\
	\midrule
		\multicolumn{2}{l}{\rowIV} & \the\numexpr\RESmcf\relax & \the\numexpr\METAmcf\relax & \the\numexpr\TOTALmcf\relax\\
	\midrule
		\multicolumn{2}{l}{\rowV} & \the\numexpr\RESmilc\relax & \the\numexpr\METAmilc\relax & \the\numexpr\TOTALmilc\relax\\
	\midrule
		\multicolumn{2}{l}{\rowVI} & \the\numexpr\RESgobmk\relax & \the\numexpr\METAgobmk\relax & \the\numexpr\TOTALgobmk\relax\\
	\midrule
		\multicolumn{2}{l}{\rowVII} & \the\numexpr\REShmmer\relax & \the\numexpr\METAhmmer\relax & \the\numexpr\TOTALhmmer\relax\\
	\midrule
		\multicolumn{2}{l}{\rowVIII} & \the\numexpr\RESsjeng\relax & \the\numexpr\METAsjeng\relax & \the\numexpr\TOTALsjeng\relax\\
	\midrule
		\multicolumn{2}{l}{\rowIX} & \the\numexpr\RESlibquantum\relax & \the\numexpr\METAlibquantum\relax & \the\numexpr\TOTALlibquantum\relax\\
	\midrule
		\multicolumn{2}{l}{\rowX} & \the\numexpr\REShref\relax & \the\numexpr\METAhref\relax & \the\numexpr\TOTALhref\relax\\
	\midrule
		\multicolumn{2}{l}{\rowXI} & \the\numexpr\RESlbm\relax & \the\numexpr\METAlbm\relax & \the\numexpr\TOTALlbm\relax\\
	\midrule
		\multicolumn{2}{l}{\rowXII} & \the\numexpr\RESsphinx\relax & \the\numexpr\METAsphinx\relax & \the\numexpr\TOTALsphinx\relax\\
	\midrule
		\multicolumn{2}{l}{\rowXIII} & \the\numexpr\RESnginx\relax & \the\numexpr\METAnginx\relax & \the\numexpr\TOTALnginx\relax\\
	
	% Bottom of the table
	\bottomrule
\end{tabular}



==> tbl/spec-gadgets.tex <==
Benchmark ----- Total Gadgets Found
------------------------------------
400.perlbench	34371
401.bzip2	1569
403.gcc		89746
429.mcf		513
433.milc	3864
445.gobmk	37999
456.hmmer	9466
458.sjeng	3110
462.libquantum	1686
464.h264ref	14456
470.lbm		394
482.sphinx3	5628

NGINX		15434
musl libc	29743


==> tbl/tbl-loc.tex <==
% Variable declarations
\newcommand{\firstColumn}{Module}
\newcommand{\secondColumn}{Lines of code}
\newcommand{\subColumnOne}{Added lines}
\newcommand{\subColumnTwo}{Deleted lines}
\newcommand{\rowOne}{LLVM}
\newcommand{\rowTwo}{Linux Kernel}
\newcommand{\rowFinal}{Total}

\begin{tabular}{cl rr}
	% Top of the table
	\toprule
		\multicolumn{2}{c}{\multirow{2}{*}{\bf \firstColumn}} & \multicolumn{2}{c}{\bf \secondColumn}\\
		\cmidrule(r){3-4} & & {\bf \subColumnOne} & {\bf \subColumnTwo} \\

	% Middle of the table
	\midrule
		\multicolumn{2}{c}{\rowOne} & \the\numexpr\llvmAdded\relax & \the\numexpr\llvmDeleted\relax\\
		\multicolumn{2}{c}{\rowTwo} & \the\numexpr\linuxAdded\relax & \the\numexpr\linuxDeleted\relax\\
		\multicolumn{2}{c}{\bf \rowFinal}   & {\bf \totalAdded} & {\bf \totalDeleted} \\

	% Bottom of the table
	\bottomrule
\end{tabular}

% Files we keep track of - for our reference
\iffalse
Beginning of the table
> LLVM FILES
0       14      LLVM6.0.0/llvm/lib/CodeGen/CodeGenPrepare.cpp
0       1       LLVM6.0.0/llvm/lib/CodeGen/CMakeLists.txt
0       1       LLVM6.0.0/llvm/lib/CodeGen/LLVMTargetMachine.cpp
0       7       LLVM6.0.0/llvm/lib/CodeGen/AsmPrinter/AsmPrinter.cpp
7       9       LLVM6.0.0/llvm/lib/Analysis/InlineCost.cpp
0       1       LLVM6.0.0/llvm/lib/MC/MCAssembler.cpp
0       8       LLVM6.0.0/llvm/lib/MC/MCObjectFileInfo.cpp
0       3       LLVM6.0.0/llvm/lib/Target/X86/X86TargetMachine.cpp
0       2405    LLVM6.0.0/llvm/lib/Target/X86/X86TrampolineASM.cpp
1       2       LLVM6.0.0/llvm/lib/Target/X86/X86ISelLowering.cpp
0       47      LLVM6.0.0/llvm/lib/Target/X86/X86AsmPrinter.h
1       10      LLVM6.0.0/llvm/lib/Target/X86/X86AsmPrinter.cpp
1       31      LLVM6.0.0/llvm/lib/Target/X86/MCTargetDesc/X86MCCodeEmitter.cpp
8       354     LLVM6.0.0/llvm/lib/Target/X86/X86MCInstLower.cpp
0       3       LLVM6.0.0/llvm/include/llvm/LinkAllPasses.h
1       4       LLVM6.0.0/llvm/include/llvm/CodeGen/MachineInstr.h
0       82      LLVM6.0.0/llvm/include/llvm/CodeGen/AsmPrinter.h
0       6       LLVM6.0.0/llvm/include/llvm/MC/MCObjectFileInfo.h
0       3       LLVM6.0.0/llvm/include/llvm/InitializePasses.h
TOTAL ADDED: 2991
TOTAL DELETED: 19
 > KERNEL FILES
9       28      linux-4.17/kernel/exit.c
0       365     linux-4.17/kernel/mardu-rerand.c
0       110     linux-4.17/kernel/mardu-ss.c
2       27      linux-4.17/kernel/fork.c
0       12      linux-4.17/kernel/sched/core.c
0       890     linux-4.17/kernel/mardu-patch.c
0       1777    linux-4.17/kernel/mardu-cr.c
0       47      linux-4.17/kernel/mardu_i.h
0       4       linux-4.17/include/asm-generic/unistd.h
0       11      linux-4.17/include/linux/syscalls.h
0       6       linux-4.17/include/linux/sched.h
0       5       linux-4.17/include/linux/fs.h
0       6       linux-4.17/include/linux/mm_types.h
0       383     linux-4.17/include/linux/mardu.h
TOTAL ADDED: 3671
TOTAL DELETED: 11
\fi


==> tbl/trampolines.tex <==
% Variable declarations
\newcommand{\firstColumn}{Benchmark}
\newcommand{\secondColumn}{Numbers of Trampolines}
\newcommand{\subColumnI}{Call Trampolines}
\newcommand{\subColumnII}{Return Trampolines}
\newcommand{\subColumnIII}{Total}
\newcommand{\rowI}{400.perlbench}
\newcommand{\rowII}{401.bzip2}
\newcommand{\rowIII}{403.gcc}
\newcommand{\rowIV}{429.mcf}
\newcommand{\rowV}{433.milc}
\newcommand{\rowVI}{445.gobmk}
\newcommand{\rowVII}{456.hmmer}
\newcommand{\rowVIII}{458.sjeng}
\newcommand{\rowIX}{462.libquantum}
\newcommand{\rowX}{464.h264ref}
\newcommand{\rowXI}{470.lbm}
\newcommand{\rowXII}{482.sphinx3}
\newcommand{\rowXIII}{NGINX}
\newcommand{\rowXIV}{Musl Libc}

\begin{tabular}{ll rrr}
	% Top of the table
	\toprule
		\multirow{2}[3]{*}{\bf \firstColumn} & \multicolumn{3}{c}{\bf \secondColumn}\\
		\cmidrule(ll){2-5} & & {\bf \subColumnI} & {\bf \subColumnII} & {\bf \subColumnIII}\\

	% Middle of the table
	\midrule
		\multicolumn{2}{l}{\rowI} & \the\numexpr\ENTRYperlbench\relax & \the\numexpr\RETperlbench\relax & \the\numexpr\TOTALperlbench\relax\\
	\midrule
		\multicolumn{2}{l}{\rowII} & \the\numexpr\ENTRYbzip\relax & \the\numexpr\RETbzip\relax & \the\numexpr\TOTALbzip\relax\\
	\midrule
		\multicolumn{2}{l}{\rowIII} & \the\numexpr\ENTRYgcc\relax & \the\numexpr\RETgcc\relax & \the\numexpr\TOTALgcc\relax\\
	\midrule
		\multicolumn{2}{l}{\rowIV} & \the\numexpr\ENTRYmcf\relax & \the\numexpr\RETmcf\relax & \the\numexpr\TOTALmcf\relax\\
	\midrule
		\multicolumn{2}{l}{\rowV} & \the\numexpr\ENTRYmilc\relax & \the\numexpr\RETmilc\relax & \the\numexpr\TOTALmilc\relax\\
	\midrule
		\multicolumn{2}{l}{\rowVI} & \the\numexpr\ENTRYgobmk\relax & \the\numexpr\RETgobmk\relax & \the\numexpr\TOTALgobmk\relax\\
	\midrule
		\multicolumn{2}{l}{\rowVII} & \the\numexpr\ENTRYhmmer\relax & \the\numexpr\REThmmer\relax & \the\numexpr\TOTALhmmer\relax\\
	\midrule
		\multicolumn{2}{l}{\rowVIII} & \the\numexpr\ENTRYsjeng\relax & \the\numexpr\RETsjeng\relax & \the\numexpr\TOTALsjeng\relax\\
	\midrule
		\multicolumn{2}{l}{\rowIX} & \the\numexpr\ENTRYlibquantum\relax & \the\numexpr\RETlibquantum\relax & \the\numexpr\TOTALlibquantum\relax\\
	\midrule
		\multicolumn{2}{l}{\rowX} & \the\numexpr\ENTRYhref\relax & \the\numexpr\REThref\relax & \the\numexpr\TOTALhref\relax\\
	\midrule
		\multicolumn{2}{l}{\rowXI} & \the\numexpr\ENTRYlbm\relax & \the\numexpr\RETlbm\relax & \the\numexpr\TOTALlbm\relax\\
	\midrule
		\multicolumn{2}{l}{\rowXII} & \the\numexpr\ENTRYsphinx\relax & \the\numexpr\RETsphinx\relax & \the\numexpr\TOTALsphinx\relax\\
	\midrule
		\multicolumn{2}{l}{\rowXIII} & \the\numexpr\ENTRYnginx\relax & \the\numexpr\RETnginx\relax & \the\numexpr\TOTALnginx\relax\\
	\midrule
		\multicolumn{2}{l}{\rowXIV} & \the\numexpr\ENTRYmusl\relax & \the\numexpr\RETmusl\relax & \the\numexpr\TOTALmusl\relax\\
	
	% Bottom of the table
	\bottomrule
\end{tabular}


